Modeling Turbulence in the Atmospheric Boundary Layer with Spectral Element and Finite Volume Methods

We present large-eddy-simulation (LES) modeling approaches for the simulation of atmospheric boundary layer turbulence that are of direct relevance to wind energy production. In this paper, we study a GABLS benchmark problem using high-order spectral element code Nek5000/RS and a block-structured second-order finite-volume code AMR-Wind which are supported under the DOE's Exascale Computing Project (ECP) Center for Efficient Exascale Discretizations (CEED) and ExaWind projects, respectively, targeting application simulations on various acceleration-device based exascale computing platforms. As for Nek5000/RS we demonstrate our newly developed subgrid-scale (SGS) models based on mean-field eddy viscosity (MFEV), high-pass filter (HPF), and Smagorinsky (SMG) with traction boundary conditions. For the traction boundary conditions, a novel analytical approach is presented that solves for the surface friction velocity and surface kinematic temperature flux. For AMR-Wind, standard SMG is used and discussed in detail the traction boundary conditions for convergence. We provide low-order statistics, convergence and turbulent structure analysis. Verification and convergence studies were performed for both codes at various resolutions and it was found that Nek5000/RS demonstrate convergence with resolution for all ABL bulk parameters, including boundary layer and low level jet (LLJ) height. Extensive comparisons are presented with simulation data from the literature.

==> tex/amr.tex <==
\section{AMR}


\begin{itemize}
 \item figures
 \item formulations
\end{itemize}
~              


==> tex/ananias_orig.tex <==
\section{Benchmark Cases and Modeling Aproaches}
%\section{All the Modeling Aproaches from Ananias}
%Nek only discussion for (2)-(7) approaches?
%   \begin{itemize}
%    \item NEK:
%        \begin{itemize}
%         \item  (7) studies with neutral flow
%
%         \item  (6) SMAG, standard approach same as AMR-Wind
%
%         \item  (5) SMAG (SGS isotropic) + MFEV (SGS anisotropic below 100m) + traction
%
%         \item  (4) SMAG (SGS isotropic) + MFEV (SGS anisotropic) + traction
%
%         \item  (3) HPF (SGS isotropic) + MFEV (SGS anisotropic) + traction
%
%         \item  (2) HPF (SGS isotropic) + traction
%
%         \item  (1) HPF + no traction
%        \end{itemize}
%
%    \item AMR-Wind: BC treament update (Matt)
%   \end{itemize}

We consider the GABLS benchmark problem~\cite{beare06} which is a stable ABL in 
which the ground temperature is cooler than the air temperature and continues to cool over the 
duration of the simulation. We investigate several SGS modeling approaches 
and wall boundary conditions as discussed below.

\subsection{ABL GABLS Benchmark}

We describe the GABLS benchmark problem~\cite{beare06}, a stable ABL 
in which the ground temperature (at $z=0$) is cooler than the air temperature and 
continues to cool over the duration of the simulation.  
We define the domain as $\Omega = L_x \times L_y \times L_z =$ 400 m $\times$ 400 m $\times$ 400 m,
with the streamwise direction $x$, the spanwise direction $y$, and  the vertical direction $z$.
We initialize our simulations at time $t=0$ with a constant velocity in the
streamwise direction equal to the geostrophic wind speed of $U=8$ m/s. We define
the initial potential temperature by 265 K in $0\le z\le 100$ m and linearly increase at
a rate of 0.01 K/m in the range of 100 m $\le z\le 400$ m.  The reference potential
temperature is 263.5 K.  The Reynolds number is $Re= UL_b/\nu$,
where $L_b=100$ m is the thickness of the initial thermal boundary layer and $\nu$ 
is the molecular viscosity, and it is $\approx 50M$, which precludes direct numerical 
simulation (DNS) wherein all turbulent scales are resolved.
We add an initial perturbation to the temperature with an amplitude of 0.1 K
on the potential temperature field for $0 \le z\le 50$ m.
%% For Nek5000/RS, this perturbation consists of a number of prime wavenumbers in the two 
%% horizontal directions (e.g., 13, 23) to mimic a small-scale random noise. A similar
%% perturbation was also tried for the three velocity components with an amplitude
%% of 0.08 m/s but the flow development was very similar to the case with only a
%% potential-temperature initial perturbation. Hence, simulations presented only had 
%% potential-temperature perturbation.

\noindent          
Periodic boundary conditions (BCs) are used in the streamwise and spanwise directions.
At the top boundary, ($z=400$ m), a stress-free, rigid lid is applied for momentum, and
the heat flux for the energy equation is set consistent with the 0.01 K/m temperature
gradient initially prescribed in the upper region of the flow.
At the bottom boundary, we perform simulations with impenetrable traction BCs
for the velocity where the specified shear stress comes from Monin-Obukhov
similarity theory~\cite{monin1954}. For the energy equation, a heat flux is
applied that is derived from the same theory and a specified potential
temperature difference between the flow at a height, $z_1$, and the surface.
The surface temperature is from the GABLS specification following the rule
$\theta_b(t) = 265 - 0.25 t$, where $t$ is in hours.  Because the boundary
conditions are periodic (lateral), or the mass flow rate through the boundaries
is zero (top and bottom),  pressure boundary conditions are not needed.

\subsection{SGS Modeling Approaches}

%\noindent
We have extended the range of our SGS modeling approaches, in the
context of the mean-field eddy viscosity approach (MFEV)~\cite{sullivan94}, to include 
the solution of an SGS turbulent kinetic energy equation (TKE). 
In our earlier ANL report~\cite{ANL22_report}, we discussed the modeling approaches for the following:

\medskip
   \begin{enumerate}[label=(\arabic*)] %%% ,noitemsep, nolistsep]
         \item   HPF SGS model + no-slip BCs
         \item   HPF SGS model + traction BCs
         \item   MFEV (SGS for anisotropic part) + HPF (SGS for isotropic) + traction BCs
         \item   MFEV (SGS for anisotropic part) + SMG (SGS for isotropic) + traction BCs
   \end{enumerate}
\medskip

\noindent
In the earlier report~\cite{ANL22_report}, two different types of boundary conditions 
were used in Nek5000/NekRS at the bottom boundary representing the lower wall. These 
boundary conditions (BCs) were no-slip and traction BCs. In this report, we consider 
only traction boundary conditions for all simulations reported, in which the normal velocity 
component was forced to zero and traction BCs were specified for the two horizontal 
velocity components; in addition, heat flux BCs were specified for the potential 
temperature, based on the Monin-Obukhov log-law~\cite{monin1954}.
%      qwall1=(dtht*cond/tplus)*factrt ! utrans


\noindent          
Results obtained with the MFEV/HPF approch led to converged results with increasing resolution.
Figure~\ref{fig.mfev_hpf_smg} (a) shows horizontally averaged profiles of streamwise and spanwise velocities
at $t=7h$, and demostrates convergence with increasing resolution from $n=128^3$ to $n=1024^3$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{./figs/nek-hpf-conv.png}
    \includegraphics[width=0.48\textwidth]{./figs/nek-mfev-conv.png}
  \end{center}
  \caption{\label{fig.mfev_hpf_smg} Nek5000 Convergence:  (a) MEFV+HPF and (b)  MFEV+SMG.}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
In addition, the obtained profiles were almost identical for different values of $Re$, as well as
of $z_1^+$ as reported in~\cite{ANL22_report}.
Results obtained with the MFEV/SMG approach also demonstrate convergence with increasing resolution
as well as asymptotic convergence with $Re$ and $z_1^+$. Moreover, convergence with resolution
seems to be faster with MFEV/SMG as compared with the MFEV/HPF approach described earlier.
This can be observed in Fig.~\ref{fig.mfev_hpf_smg} (b), which shows horizontally averaged streamwise and 
spanwise velocities at $t=7h$ using MFEV/SMG and traction boundary conditions. 

\noindent
Interestingly, the difference between the mean profiles obtained with MFEV/HPF and MFEV/SMG is reduced
with increasing resolution as can be observed in Figs.~\ref{fig.plot_MFEV_HPF_SMG} (a)--(c).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*} [!t]
  \begin{center}
    \includegraphics[width=0.5\textwidth]{./figs/plot_MFEV_HPF_SMG_128.pdf}
    \hspace{-2em}
    \includegraphics[width=0.5\textwidth]{./figs/plot_MFEV_HPF_SMG_256.pdf}
    \\
    \vspace{-2em}
    \includegraphics[width=0.5\textwidth]{./figs/plot_MFEV_HPF_SMG_512.pdf}
  \end{center}
  \caption{\label{fig.plot_MFEV_HPF_SMG} 
   Comparison between mean profiles obtained with MEFV+HPF and MFEV+SMG with 
   resolution (a) $n=128^3$, (b) $n=256^3$ and (c) $n=512^3$.}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
Figure~\ref{fig.nek-amr-512} (a) shows the horizontally averaged streamwise and spanwise velocities and Fig.~\ref{fig.nek-amr-512}(b) the 
horizontally averaged potential temperature at t=6h for the two highest resolutions $512^3$ and $1024^3$ for MFEV/HPF and for $512^3$ 
for MFEV/SMG and AMR-Wind, respectively. As can be observed, both Nek5000/NekRS converge to the same profiles as resolution is increased; 
they also agree well with the AMR-Wind obtained profiles at $512^3$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{./figs/nek-amr-512.png}
    \includegraphics[width=0.48\textwidth]{./figs/nek-amr-temp-512.png}
  \end{center}
  \caption{\label{fig.nek-amr-512} Horizontally averaged (a) streamwise, spanwise velocities and (b) potential temperature at t=6h using MFEV/SMG and MFEV/HPF
      with traction boundary conditions, compard with AMR-Wind results, for $512^3$.}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
Figures~\ref{fig.nek-amr-hr} (a)--(d) show horizontally averaged streamwise and spanwise velocity profiles at different times
$t=6h$, $t=7h$, $t=8h$ and $t=9h$, demonstrating good agreement between MFEV/HPF, MFEV/SMG and AMR-Wind, for $n=512^3$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{./figs/nek-amr-6h.png}
    \includegraphics[width=0.48\textwidth]{./figs/nek-amr-7h.png}
    \\
    \includegraphics[width=0.48\textwidth]{./figs/nek-amr-8h.png}
    \includegraphics[width=0.48\textwidth]{./figs/nek-amr-9h.png}
  \end{center}
  \caption{\label{fig.nek-amr-hr} Mean velocity profiles from Nek5000 MEFV+HPF, MFEV+SMG, and AMR-Wind SMG at (a) $t=6h$, (b) $t=7h$, (c) $t=8h$, and (d) $t=9h$.}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent
Here, we focus primarily on the approaches that are based on an SGS TKE equation as follows:
%used for this benchmark problem based on high-pass filter (HPF)~\cite{Stolz_Schlatter_2005}, 
%and Smagorinsky (SMG)~\cite{smagor63} with no-slip and traction BCs summarized as:

\medskip
   \begin{enumerate}[label=(\arabic*),noitemsep, nolistsep]
    \setcounter{enumi}{5}
         \item   MFEV (SGS for anisotropic part) + SGS TKE (SGS for isotropic part) + $L_{SMG}$
         \item   MFEV (SGS for anisotropic part) + SGS TKE (SGS for isotropic part) + $L_{DRD}$
   \end{enumerate}
\medskip

\noindent
The SGS TKE equation and the definition of the length scales $L_{SMG}$ and $L_{DRD}$ are described 
in the following.
In addition to the above, sampling for the evaluation of the wall momentum and heat fluxes was
extended to include specified $z-$locations away from the lower wall.

\subsubsection{MFEV (SGS for anisotropic part) + SGS TKE (SGS for isotropic) + traction BCs}
\label{sec.mfev_sgstke}
In the efforts described in this subsection, the traction BCs for the horizontal velocity 
components is implemented in the context of the log-law for which we follow the approach of ~\cite{Grotjans_Menter1998} 
and~\cite{Kuzmin_2007}, which is suitable for finite element methods based on a weighted residual formulation.
The normal component of the velocity is set to zero and the traction BCs imposed on the tangential velocity are based 
on the horizontally-averaged slip velocity that develops at the boundary or at a specified sampling $z-$location
from the lower wall.


\noindent
The SGS modeling is based on~\cite{sullivan94}, where the SGS stress tensors $\tau^{sgs}_{ij}$ and $\tau^{sgs}_{\theta j}$ 
are expressed in terms of a non-isotropic and an isotropic part. Thus, the sub-grid-scale dissipation is based on a 
non-isotropic, MFEV $\nu_T$ obtained by the horizontally-averaged mean strain rate, and an isotropic, 
fluctuating part $\nu_t$, which is a function of the SGS TKE obtained from a transport equation as desctibed below.
The law of the wall is effected through the use of the MFEV concept and the approach originally used 
by~\cite{SCHUMANN1975376} is used to convert the horizontally-averaged traction to local values based on the local slip velocity 
in each of the horizontal directions. The SGS model of~\cite{sullivan94} is based on the following expression
\begin{equation}
\tau^{sgs}_{i j}=-2 \gamma \nu_t S_{i j} -2 \nu_{T}\left\langle S_{i j}\right\rangle,
\label{eqn.tijdef2}
\end{equation}
\noindent
where $\left\langle \ \ \right\rangle$ denote averaging over the
homogeneous directions and $\nu_T$ is an average eddy viscosity which is expressed in
terms of mean flow quantities. In Eq.~(\ref{eqn.tijdef2}) $\gamma$ is
an ``isotropy factor,'' which accounts for variability in the SGS constants due to
anisotropy of the mean flow. The fluctuating eddy viscosity, $\nu_t$, is obtained from the SGS turbulent 
kinetic energy equation, in which the shear production term is computed 
from the fluctuating velocities as suggested by~\cite{Schumann1975}. When the fluctuating (isotropic) part of 
turbulent motion is taken into account through the use the fluctuating strain rate, $\nu_t$ in Eq.~(\ref{eqn.tijdef2}) 
is non-zero and the full stress tensor has to be taken into account. Thus, the momentum and potential temperature 
equations are given by

\begin{eqnarray}
 \label{eq:ns3}
  \frac{\partial \bar{u}_{i}}{\partial t}
  +\bar{u}_{j}\frac{\partial \bar{u}_{i}}{\partial x_{j}}
  & = & -\frac{\partial \bar{p}}{\partial x_{i}}-\pp{\tau_{ij}}{x_j}
        -2 \epsilon_{i3k} \Omega \bar{u}_k %%\nonumber \\
    +  (1-\delta_{i3}) \frac{\partial }{\partial z}\nu_{T} 
   \frac{\partial\langle \bar{u}_i\rangle}{\partial z} - \frac{\theta^{\prime}}{\theta_0} g_i \quad  \\ %\label{eq:inc_filt}
  & = & -\frac{\partial \bar{p}}{\partial x_{i}}
        + \frac{\partial}{\partial x_j} \left(\frac{1}{\operatorname{Re}} +\gamma \nu_t \right) 
          2S^n_{ij} - 2 \epsilon_{i3k} \Omega \bar{u}_k %%\nonumber\\
    +   (1-\delta_{i3}) 
      \frac{\partial }{\partial z}\nu_{T} \frac{\partial\langle \bar{u}_i \rangle}{\partial z} - \frac{\theta^{\prime}}{\theta_0} g_i, \quad
\\
%\end{eqnarray} \label{eq:inc_filt3}
%\begin{eqnarray}
  \frac{\partial \bar{\theta}}{\partial t}
  + \bar{u}_{j}\frac{\partial \bar{\theta}}{\partial x_{j}}
  %&=& -\pp{\tau_{\theta j}}{x_j} \\
    \label{eq:energy_filt3}
  & = & \frac{\partial }{\partial x_{j}} \left(\frac{1}{\operatorname{Pe}}
   +\frac{\gamma \nu_t}{Pr_t} \right) \frac{\partial \bar{\theta}}{\partial x_{j} }
   + \frac{\partial }{\partial z}\nu_{T} \frac{\partial\langle \bar{\theta} \rangle}{\partial z}.
\end{eqnarray}

\noindent
The transport equation for the subgrid scale turbulent kinetic energy equation~\cite{sullivan94} is:

\begin{equation}
\left(\frac{\partial}{\partial t}+u_j \frac{\partial}{\partial x_j}\right) e =2 \gamma \nu_t S^{\prime}_{i j} S^{\prime}_{i j} + \frac{g}{\theta_0} \tau_{\theta w} -C_\varepsilon \frac{e^{3 / 2}}{L}+\frac{\partial}{\partial x_i} \left(\frac{1}{\operatorname{Re}} +2 \gamma \nu_t \right) \frac{\partial e}{\partial x_i} \\
%\nu_\theta=\left(1+\frac{2 l}{\Delta}\right) \nu_t \quad B & =\frac{g}{\theta_0} \tau_{\theta w} \quad \tau_{\theta i}=-\nu_\theta \frac{\partial \theta}{\partial x_i}
\end{equation}

\noindent
and the fluctuating eddy viscosity, $\nu_t$, is given by
\[\nu_t=C_k L e^{1 / 2}.\]

\noindent
For unstable stratification the length scale $L$ in this equation becomes 
\[L_{SMG}=\Delta,\]

\noindent
while for stable stratification, $L$ is reduced as suggested by~\cite{deardorff80} and is obtained by the following expression
\[L_{DRD}=\frac{0.76 e^{1 / 2}}{\left(\frac{g}{\theta_0} \frac{\partial \theta}{\partial z}\right)^{1 / 2}}.\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{./figs/nek-tke-smg-z-z0-10-7h.png}
  \end{center}
  \caption{\label{fig.nek-tke-smg} Nek5000 Convergence: MEFV+SMG and MFEV+HPF.}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
The definition of $\tau_{\theta w}$ is
\[\quad \tau_{\theta w}=-\nu_\theta \frac{\partial \theta}{\partial z},\]

\noindent
whereas 
\[C_{\varepsilon}=0.19+0.74 L / \Delta,\]

\noindent
and $S^{\prime}_{i j}$ is given by

\[ S^{\prime}_{i j} = S_{i j}-\left\langle S_{i j}\right\rangle.\]

\noindent
The Smagorinsky constant $C_s$ is written in terms of $C_k$ and $C_{\varepsilon}$
\[C_s=\left(C_k \sqrt{\frac{C_k}{C_\varepsilon}}\right)^{1 / 2}.\]

\noindent
From~\cite{sullivan94}, the SGS constants are $C_k = 0.1$ and for the case where 
$L=L_{SMG}=\Delta$, $C_{\varepsilon}=0.93$.  The isotropy factor $\gamma$ is obtained from
\begin{equation}
\gamma=\frac{S^{\prime}}{S^{\prime}+\langle S\rangle},
\end{equation}

\noindent
where
\begin{equation}
\langle S\rangle=\sqrt{2\left\langle S_{i j}\right\rangle\left\langle S_{i j}\right\rangle},
\end{equation}

\noindent
and
\begin{equation}
S^{\prime}=\sqrt{2 \left\langle S^{\prime}_{i j} S^{\prime}_{i j} \right\rangle}.
\end{equation}

%$\begin{aligned}
%& \epsilon=C_\epsilon \frac{e^{3 / 2}}{l} \\
%& l=\frac{0.76 e^{1 / 2}}{\left(\frac{g}{\theta_0} \frac{\partial \theta}{\partial z}\right)^{1 / 2}}
%\end{aligned}$
%$\nu_t=C_k l e^{1 / 2}$
%$P=2 \nu_t \gamma\left(S_{i j}-\left\langle S_{i j}\right\rangle\right)\left(S_{i j}-\left\langle S_{i j}\right\rangle\right)$
%l=\Delta=L_e / N
%$D=\frac{\partial}{\partial x_i}\left(2 \nu_t \frac{\partial e}{\partial x_i}\right)$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{./figs/nek-pr1-128.png}
    \includegraphics[width=0.48\textwidth]{./figs/nek-pr1-256.png}
    \\
    \includegraphics[width=0.48\textwidth]{./figs/nek-pr1-512.png}
  \end{center}
  \caption{\label{fig.nek-pr1_z10_z50} Effect of sampling location: horizontally averaged streamwise and spanwise velocity profiles at $t=7h$ using
$z_{smpl}/z_0$ values between 10 and 50 for resolutions (a) $n=128^3$, (b) $n=256^3$, and (c) $n=512^3$.}
\end{figure*}

\noindent
The expression for the MFEV $\nu_T$ is derived so that the law-of-the-wall behavior
can be recovered in the absence of any resolved turbulence as explained below.
According to~\cite{sullivan94}, a model consistent with this idea is as follows:
\begin{equation}
\nu_{T}=\left(C_{K} L_{m}\right)^{2} \sqrt{2\left\langle S_{i j}\right\rangle\left\langle S_{i j}\right\rangle},
 \label{eqn.nuT1}
\end{equation}
where $S_{i j}$ is the strain rate tensor, $C_K$ is a constant and $C_K L_m$ is a mixing-lqength scale.
Equation~(\ref{eqn.nuT1}) simplifies to
\begin{equation}
\nu_{T}=\left(C_{K} L_{m}\right)^{2} \sqrt{\left(\frac{\partial\langle u\rangle}{\partial z}\right)^{2}+\left(\frac{\partial\langle v\rangle}{\partial z}\right)^{2}},
\label{eqn.nuT2}
\end{equation}
\noindent
and by ignoring the mean wind turning with height at the first grid point implies that the
wind-speed derivative is:
\begin{equation}
\sqrt{\left(\frac{\partial\langle u\rangle}{\partial z}\right)^{2}+\left(\frac{\partial\langle v\rangle}{\partial z}\right)^{2}} \approx \frac{\partial U_{s}}{\partial z},
\label{eqn.dUdz1}
\end{equation}
\noindent
where $U_{s}$ is the average surface layer wind speed (i.e., $U_{s}=\left\langle\sqrt{u^{2}+v^{2}}\right\rangle$).
The choice of $C_K L_m$ is guided by the need to match Monin-Obukhov similarity theory in the
wall region and the expression. In this theory, the wind-speed derivative becomes
\begin{equation}
\frac{\partial U_{s}}{\partial z}=\frac{u_{\tau} \phi_{m}}{\kappa z},
\label{eqn.dUdz2}
\end{equation}
where $u_{\tau}$ is the friction velocity, $\kappa$ the von Karman constant, $\phi_{m}$ the Monin-Obukhov stability
function for momentum.
Following~\cite{sullivan94}, in order to make use of Equation~(\ref{eqn.nuT1}) we further impose a ``constant flux'',
traction-type boundary condition at $z=z_{1}$, which states that the sum of the SGS and resolved momentum fluxes be
equal to the surface stress, i.e.,
\begin{equation}
\left[\left\langle\tau^{sgs}_{u w}\right\rangle^{2}+\left\langle\tau^{sgs}_{v w}\right\rangle^{2}\right]^{1 / 2}
 +\left[\langle u w\rangle^{2}+\langle v w\rangle^{2}\right]^{1 / 2}=u_{\tau}^{2} .
\label{eqn.stress}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{./figs/nek-var-pr-conv-z-z0-10.png}
    \includegraphics[width=0.48\textwidth]{./figs/nek-var-pr-conv-z-z0-50.png}
  \end{center}
  \caption{\label{fig.nek-var-pr-conv-z10-z50} Effect of $Pr_t$: horizontally averaged streamwise and spanwise velocity profiles at $t=7h$ at resolutions
$128^3$, and $256^3$, using (a) $z_{smpl}/z_0=10$ and (b) $z_{smpl}/z_0=50$, with $Pr_t$ taking values $1$ and $1/3$.}
\end{figure*}
%%%%%%%%%
\noindent
As described in section~\cite{ANL22_report}, this traction boundary condition in Nek is imposed at the
first grid point in the vertical direction, which is assumed to be a point inside the log-layer at a location $z=z_1$,
where the boundary condition for the vertical velocity component is defined to be zero.
For this reason the second term in equation~(\ref{eqn.stress}) corresponding to the resolved momentum fluxes is
identically equal to zero.
\noindent
In~\cite{sullivan94}, a predictive relationship for the mean-field eddy-viscosity
at the first grid point $z_1$, $\nu_T^\star=\nu_T(z_1)$, is obtained by invoking the approximation
that the fluctuating components of strain are neglected compared to the mean strain so
that only the horizontally-averaged SGS stress in Eq.~(\ref{eqn.tijdef2}) is retained.
This leads to
\begin{equation}
\begin{aligned}
%\left\langle\tau_{u w}\right\rangle &=-\left(\left\langle\nu_{t} \gamma\right\rangle+\nu_{T}\right) \frac{\partial\langle u\rangle}{\partial z} \\
%\left\langle\tau_{v w}\right\rangle &=-\left(\left\langle\nu_{t} \gamma\right\rangle+\nu_{T}\right) \frac{\partial\langle v\rangle}{\partial z}
\left\langle\tau^{sgs}_{u w}\right\rangle &=-\nu_{T} \frac{\partial\langle u\rangle}{\partial z}, \\ 
\left\langle\tau^{sgs}_{v w}\right\rangle &=-\nu_{T} \frac{\partial\langle v\rangle}{\partial z}.
\label{eqn.tijsim}
\end{aligned}
\end{equation}
\noindent
Upon substitution of Eq.~(\ref{eqn.tijsim}) into Eq.~(\ref{eqn.stress}) and making use of Eqs.~(\ref{eqn.dUdz1})--(\ref{eqn.dUdz2}), the expression for the mean-field eddy-viscosity, $\nu_T^\star$, for Nek
becomes
\begin{equation}
%\nu_{T}^{\star}=\frac{u_{\tau} \kappa z_{1}}{\phi_{m}\left(z_{1}\right)}-\left\langle\nu_{t} \gamma\right\rangle-\frac{\kappa z_{1}}{u_{\tau} \phi_{m}\left(z_{1}\right)}\left[\langle u w\rangle^{2}+\langle v w\rangle^{2}\right]^{1 / 2}
\nu_{T}^{\star}=\frac{u_{\tau} \kappa z_{1}}{\phi_{m}\left(z_{1}\right)}.
\label{eqn.nuTsim}
\end{equation}

\noindent
Equation~(\ref{eqn.nuTsim}) provides an adaptive method for estimating the mean-field eddy
viscosity needed to force the computed wind speed derivative to match with
similarity theory at $z = z_1$. At any other height, similar to~\cite{sullivan94}, we use
\begin{equation}
\nu_{T}=\nu_{T}^{\star} \frac{\kappa z_{1}}{u_{\tau} \phi_{m}\left(z_{1}\right)} \sqrt{2\left\langle S_{i j}\right\rangle\left\langle S_{i j}\right\rangle},
 \end{equation}
\noindent
which follows directly from Eqs.~(\ref{eqn.nuT1}), ~(\ref{eqn.dUdz1}), and~(\ref{eqn.dUdz2}).
In contrast to~\cite{sullivan94}, a similar correction was also applied to the SGS potential temperature
field, and $\tau^{sgs}_{\theta z}$ becomes:
\begin{equation}
\left\langle\tau^{sgs}_{\theta z}\right\rangle =-\nu_{T} \frac{\partial\langle \theta \rangle}{\partial z}.
\label{eqn.tautheta}
\end{equation}
\noindent

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
  \begin{center}
    \includegraphics[width=0.5\textwidth]{./figs/plot_mean_prof_128_7h_MFEV_sgstkePrt1_vs_deard_zsmpl10.pdf}
    \hspace{-2em}
    \includegraphics[width=0.5\textwidth]{./figs/plot_mean_prof_256_7h_MFEV_sgstkePrt1_vs_deard_zsmpl10.pdf}
    \\
    \vspace{-2em}
    \includegraphics[width=0.5\textwidth]{./figs/plot_mean_prof_512_7h_MFEV_sgstkePrt1_vs_deard_zsmpl10.pdf}
  \end{center}
  \caption{\label{fig.plot_mean_prof_mfev_sgstkePrt1_vs_deard_zsmpl10} Effect of $L_{SMG}$ vs $L_{DRD}$ on horizontally averaged streamwise and
spanwise velocity profiles at $t=7h$ for resolutions (a) $n=128^3$, (b) $n=256^3$, and (c) $n=512^3$ using MFEV/SGS-TKE and $L_{SMG}$ vs $L_{DRD}$.}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Traction BCs
%The implementation of this boundary
%condition in Nek5000/RS is performed using the full stress formulation~\cite{LeeHo1989} and allows also for
%boundaries that are curved and not alligned with any of the axes. The evaluation of the local momentum flux used
%for the traction BCs is described in detail in Section~\ref{s:tractionBC}.
\noindent
Following~\cite{Grotjans_Menter1998} and~\cite{Kuzmin_2007}, as was already described in the previous subsection, in our approach 
the boundary of the computational domain
is not located exactly at the wall but at a finite distance from the wall corresponding to a fixed value of $z_1^+=z/z_0$.
Strictly speaking, this implies that a boundary layer of width $z_1$ (corresponding to the specified value of $z_1^+$) should
be removed from the computational domain; however, it is assumed that this width is very small at high Reynolds numbers
and can be considered negligible, so that the equations can be solved in the whole domain with traction BCs prescribed
on the lower boundary. Since the choice of $z_1^+$ is rather arbitrary, we have found that values of $z_1^+$ up
to $10$ at the target $Re$ produce averaged results that do not differ significantly.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{./figs/nek-stat-128.png}
    \includegraphics[width=0.48\textwidth]{./figs/nek-stat-256.png}
    \includegraphics[width=0.48\textwidth]{./figs/nek-stat-512.png}
  \end{center}
  \caption{\label{fig.plot_fluc_mfev_sgstkePrt1_vs_deard_zsmpl10} Effect of $L_{SMG}$ vs $L_{DRD}$ on horizontally averaged streamwise,
spanwise and normal fluctuation profiles at $t=7h$ for resolutions (a) $n=128^3$, (b) $n=256^3$, and (c) $n=512^3$ using MFEV/SGS-TKE and $L_{SMG}$ vs $L_{DRD}$.}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Results with MFEV/SGS-TKE}
%\noindent
This section presents results obtained with the mean-field eddy viscosity approach 
(MFEV) in conjunction with solving a SGS turbulent kinetic energy equation (TKE).
Figure~\ref{fig.nek-tke-smg} compares horizontally averaged streamwise and spanwise velocity
profiles at $t=7h$, using MFEV/SMG and MFEV/SGS-TKE with $L_{SMG}$ for resolutions $n=128^3$, $n=256^3$ and $n=512^3$. 
For completeness, the MFEV/HPF profiles for $n=1024^3$ are also shown. As can be observed, the difference between
MFEV/SMG and MFEV/TKE-SMG using $L_{SMG}$ is negligible for all resolutions.

\noindent
As noted earlier, here we extended the work of the earlier report~\cite{ANL22_report} by allowing for the sampling
of tangential velocities and potential temperature at specified $z-$locations away from the lower wall in order to
evaluate $u_{\tau}$ and $\theta_{\tau}$, i.e. the wall momentum and heat fluxes. The evaluation of $u_{\tau}$ and $\theta_{\tau}$
is performed using the system of equations and method presented in section 4 of~\cite{ANL22_report}. To investigate the effect of the 
sampling location $z_{smpl}$ on the results, simulations using MFEV/SGS-TKE with $L_{SMG}$ were performed 
for various values of $z_{smpl}/z_0$ ranging between 10 and 50, for various resolutions. Figure~\ref{fig.nek-pr1_z10_z50} 
shows horizontally averaged streamwise and spanwise velocity profiles at $t=7h$ using $z_{smpl}/z_0$ values between 10 
and 50 for resolutions (a) $n=128^3$, (b) $n=256^3$, and (c) $n=512^3$. An important conclusion from this study was that
the effect of the sampling location diminishes with resolution and already at $n=512^3$ it is almost negligible.

\noindent
The effect of $Pr_t$ was also investigated for the case MFEV/SGS-TKE with $L_{SMG}$ and the results are shown in 
Fig.~\ref{fig.nek-var-pr-conv-z10-z50} (a) and (b) at resolutions $n=128^3$, and $n=256^3$, with $Pr_t$ taking values $1$ and $1/3$
for $z_{smpl}/z_0=10$ and $z_{smpl}/z_0=50$, respectively. As can be observed, the effect of $Pr_t$ is almost negligible for both resolutions studied.


\noindent
A comparison of the horizontally averaged streamwise and spanwise velocity profiles at $t=7h$ between the MFEV/SGS-TKE with $L_{SMG}$ and the 
MFEV/SGS-TKE with $L_{DRD}$ approaches is shown in Fig.~\ref{fig.plot_mean_prof_mfev_sgstkePrt1_vs_deard_zsmpl10} (a)--(c) for resolutions
$n=128^3$, $n=256^3$ and $n=512^3$, respectively.

\noindent
A comparison of fluctuation velocities at $t=7h$ between the MFEV/SGS-TKE with $L_{SMG}$ and the MFEV/SGS-TKE with $L_{DRD}$ approaches is 
shown in Fig.~\ref{fig.plot_fluc_mfev_sgstkePrt1_vs_deard_zsmpl10}(a), (b) and (c) for resolutions
$n=128^3$, $n=256^3$ and $n=512^3$, respectively.


\noindent
Figure~\ref{fig.mean_sgstke_vs_deard_z10_z50} shows a comparison of the horizontally averaged streamwise and spanwise velocity profiles at $t=7h$ 
for (a) $z_{smpl}/z_0=10$ and (b) $z_{smpl}/z_0=50$, using MFEV/SGS-TKE with $L_{SMG}$ and MFEV/SGS-TKE with $L_{DRD}$ for resolutions $n=128^3$, 
$n=256^3$, and $n=512^3$. For completeness, the MFEV/HPF profiles for $n=1024^3$ are also shown.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{./figs/nek-tke-smg-drd-z-z0-10-7h.png}
    \includegraphics[width=0.48\textwidth]{./figs/nek-tke-hpf-z-z0-50-7h.png}
  \end{center}
  \caption{\label{fig.mean_sgstke_vs_deard_z10_z50} Horizontally averaged streamwise and spanwise velocity profiles at $t=7h$ for resolutions 
$n=128^3$, $n=256^3$, and $n=512^3$ using MFEV/SGS-TKE and $L_{SMG}$ vs $L_{DRD}$ for (a) $z_{smpl}/z_0=10$ and (b) $z_{smpl}/z_0=50$.}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
  \begin{center}
    \includegraphics[width=0.48\textwidth]{./figs/nek-stat-pr1-conv.png}
    \includegraphics[width=0.48\textwidth]{./figs/nek-stat-pr2-conv.png}
  \end{center}
  \caption{\label{fig.fluc_sgstke_vs_deard_z10_z50} horizontally averaged streamwise, spanwise and normal fluctuation profiles at $t=7h$
for $z_{smpl}/z_0=10$ using (a) MFEV/SGS-TKE with $L_{SMG}$ and (b) MFEV/SGS-TKE with $L_{DRD}$ for resolutions $n=128^3$, $n=256^3$, and $n=512^3$.}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}%[!t]
  \begin{center} 
    \includegraphics[width=0.47\textwidth]{./figs/nek5_spectrum.png}
    \includegraphics[width=0.49\textwidth]{./figs/plot_L_Obukhov_ncarBC_all.pdf}
    \\
    \includegraphics[width=0.49\textwidth]{./figs/plot_surface_momflux_ncarBC_all.pdf}
    \includegraphics[width=0.49\textwidth]{./figs/plot_surface_heatflux_ncarBC_all.pdf}
  \end{center}
  \caption{\label{nekrs_mesh_conv4} Nek5000 spatial spectrum, Obukhov length, and
            time history of heat and momentum fluxes.} %%% this is using no-slip BC
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent
Figure~\ref{fig.fluc_sgstke_vs_deard_z10_z50} shows a comparison of the horizontally averaged streamwise, spanwise and normal fluctuation profiles at $t=7h$ 
for $z_{smpl}/z_0=10$ using (a) MFEV/SGS-TKE with $L_{SMG}$ and (b) MFEV/SGS-TKE with $L_{DRD}$ for resolutions $n=128^3$, $n=256^3$, and $n=512^3$.


\noindent
Good convergence is also observed in second order quantities in Fig.~\ref{fig.fluc_sgstke_vs_deard_z10_z50} (a) and (b),
for MFEV/SGS-TKE with (a) $L_{SMG}$ and with (b) $L_{DRD}$. This is especially the case for resolutions $n=256^3$ and $n=512^3$ and for 
$L_{SMG}$. The resolved fluctuations obtained by the two approaches MFEV/SGS-TKE+with $L_{SMG}$ and $L_{DRD}$ compare reasonably well
for the same effective resolution.
%Finally, according to~\cite{sullivan94}, the mean-field eddy viscosity $\nu_T$ and isotropy factor $\gamma$ play important 
%roles near the lower wall where mean shear is large. Away from the wall in the middle of the ABL, the fluctuating resolved 
%strain should be almost a factor of 10 larger than the mean strain for typical grid resolutions used. In this region, 
%$\nu_T \ll \nu_t$ and $\gamma \rightarrow 1$. For this reason, they suggest that for $z > z_i/2$, where $zi$ is the depth of 
%the ABL ($\approx 200$), $\gamma$ should be set to $1$ and $\nu_T$ to 0. Forcing this at lower resolutions, e.g. for $256^3$ 
%removes a bump which appears in the streamwise fluctuation profile between $z=100$ and $200$, as can be seen in 
%Fig.~\ref{fig.fluc_sgstke_vs_deard_z10_z50}.

\noindent
Figure~\ref{nekrs_mesh_conv4} (top left) demonstrates the spatial spectrum for
velocity magnitude at 6 hours for $n=256^3$ and $n=512^3$ resolutions.  We see that
both the $n=512^3$ and $n=1024^3$ results exhibit $k^{-\frac{5}{3}}$ energy
spectrum, as expected for resolved turbulent flow simulations.
The remaining figures show the comparison of Nek5000/RS to the NCAR, IMUK,
and MO results for the Monin-Obukhov length, the surface momentum flux, and
the surface heat flux.




==> tex/codes.tex <==

\section{Nek5000/RS}
Our modeling approaches are implemented into Nek5000/RS.
Nek5000~\cite{nek5000} is a spectral element code that is used for a wide range 
of thermal-fluids applications. Nek5000 has scaled to millions of MPI ranks using 
the Nek-based gsLib communication library to handle all near-neighbor and other 
stencil type communications~\cite{fischer15}.
On CPUs, tensor contractions constitute the principal computational kernel 
(typically $>$ 90\% of the flops). These can be cast as small dense matrix-matrix 
products resulting in high performance with a minor amount of tuning.

Nek5000 employs high-order spectral elements (SEs) \cite{pat84} in which the solution, 
data, and test functions  are represented as {\em locally structured} $N$th-order 
tensor product polynomials on a set of $E$ {\em globally
unstructured} curvilinear hexahedral brick elements.   The approach yields two
principal benefits.  First, for smooth functions such as solutions to the
incompressible NS equations, high-order polynomial expansions yield exponential
convergence with approximation order, implying a significant reduction in the
number of unknowns ($n \approx EN^3$) required to reach engineering tolerances.
Second, the locally structured forms permit local lexicographical ordering with
minimal indirect addressing and, crucially, the use of tensor-product sum
factorization to yield low $O(n)$ storage costs and $O(nN)$ work complexities
\cite{sao80}.  As we demonstrate, the leading order $O(nN)$ work terms can be
cast as small dense matrix-matrix products (tensor contractions) with favorable
$O(N)$ work-to-storage ratios (computational intensity)  \cite{dfm02}.

Time integration in Nek5000/RS is based on a semi-implicit splitting scheme
using $k$th-order backward differences (BDF$k$) to approximate the time
derivative coupled with implicit treatment of the viscous and pressure
terms and $k$th-order extrapolation (EXT$k$) for the remaining advection and forcing
terms.  This approach leads to independent elliptic subproblems comprising a
Poisson equation for the pressure, a coupled system of Helmholtz equations for
the three velocity components, and an additional Helmholtz equation for the
potential temperature.
The pressure Poisson equation is obtained by taking the
divergence of the momentum equation and forcing $\frac{\partial u_i^n}{\partial
x_i}=0$ at time $t^n=n \Delta t$. The velocity and temperature
Helmholtz equations are obtained once $p^n$ is known:
\begin{eqnarray} \label{pres}
-\frac{\partial^2}{\partial x_j\partial x_j} p^n\! &=&\! q^n, 
\\ \label{vel}
\frac{\beta_0}{\dt} u_i^n 
-\pp{}{x_j}\left(\frac{1}{Re}+\gamma \nu_t \right) 2S^n_{ij}
                              \! &=&\! - \pp{}{x_i} p^n + r_i^n, 
\\ \label{temp}
\hspace*{-.1in}
\left[\frac{\beta_0}{\dt} -\pp{}{x_j}\left(\frac{1}{Pe}+ 
   \frac{\gamma \nu_t}{Pr_t}\right) \pp{}{x_j}\right] \theta^n \! &=&\!  s^n,
\end{eqnarray}
where $\beta_0$ is an order-unity constant associated with BDF$k$
\cite{fischer17}, $S_{ij}$ is the resolved-scale strain-rate tensor as
described in~(\ref{eqn.tauij}), and $q^n$, $r_i^n$, and $s^n$ represent the sum
of the values from the previous timesteps for the contributions from BDF$k$ and
EXT$k$.  Also included in $r_i^n$ and $s^n$ are eddy-diffusivity terms coming
from the mean-field eddy-diffusivity mentioned above.  The fully coupled system
of Helmholtz equations for the three velocity components~(\ref{vel}) is used
only when the fluctuating (isotropic) part of the SGS stress tensor is modeled
using a Smagorinsky (SMG) model based on the fluctuating strain rate. When this
part is modeled through the use of a high-pass filter
(HPF)~\cite{Stolz_Schlatter_2005} the resulting Helmholtz equations for the
three velocity components are not coupled.

With the given time-splitting, we recast (\ref{pres})--(\ref{temp}) into weak
form and derive the spatial discretization by restricting the trial and test
spaces to be in the finite-dimensional space spanned by the spectral element
basis.   The discretization leads to a sequence of symmetric positive definite
linear systems for pressure, velocity, and temperature.  Velocity and temperature
are diagonally dominant and readily addressed with Jacobi-precondition conjugate
gradient iteration.  The pressure Poisson solve is treated with GMRES using
$p$-multigrid as a preconditioner.  Details of the formulation can be found in
\cite{fischer04,fischer17,malachi2022a}.

%Nek5000 is a computational fluid dynamics code that simulates unsteady incompressible
%fluid flow with thermal and passive scalar transport. It can handle general two- and
%three-dimensional domains described by isoparametric quad or hex elements. 
%In addition, it can be used to compute axisymmetric flows. 

NekRS supports several features to accelerate performance, including overlapped
communication and computation during operator evaluation, which yields a
10--15\% performance gain for NS simulations; FP32 local-operator inversion and
residual evaluation for the Chebyshev-accelerated Schwarz-based $p$-multigrid;
and projection of the velocity and pressure solutions onto the space
of prior solutions to generate an initial guess, which can yield
a 1.5--2-fold NS performance gain~\cite{fisc98}.
On the NVIDIA A100, the OCCA-based kernels are close to the bandwidth-limited
roofline and are sustaining 2.1--2.2 TFLOPS (FP64) for the Poisson operator,
and 3.1--3.8 TFLOPS (FP64) for the advection operator.
  In the pressure preconditioner, the forward Poisson operator on the coarser
multigrid levels realizes 2.5--3.9 TFLOPS (FP32) and the Schwarz smoother
sustains 2.5--5.1 TFLOPS (FP32).  (The lower values are for smaller values of
$N$ that are used in the $p$-multigrid V-cycle.)   Comparable values are realized
on the NVIDIA V100s on Summit, save that they are $\approx$ 1.5 times lower
than those on the A100.
Sustained flop rates for the full NS solver are $\approx 470$ GFLOPS
per V100 on Summit~\cite{nekrs,min-sc22}.

In~\cite{min-ijhpca24}, we provide detailed analysis of the GABLS benchmark performance 
on the Oak Ridge Leadership Facility supercomputers Summit, using 4 to 800 nodes 
(24 to 4,800 NVIDIA V100 GPUs), and Crusher, the testbed for the Frontier exascale 
system using 18 to 384 Graphics Compute Dies on AMD MI250X GPUs.
We also demonstrate the performance comparison of two open-source CFD codes, 
NekRS (high-order, unstructured-grid, spectral element method) and 
AMR-Wind (block-structured, second-order finite-volume method with adaptive-mesh-refinement),
provided with strong- and weak-scaling capabilities, linear solver performance, and time to solution. 
 






==> tex/convergence.tex <==
 

 \subsection{Convergence}

 -- Ananias ?

 -- Matt?     


==> tex/nek.tex <==

\section{NEK}

\begin{itemize}
 \item figures
 \item formulations
\end{itemize}


==> tex/neutral.tex <==

\section{ABL neutral benchmark}
This section presents a benchmark problem from~\cite{owen2019} corresponding to a large-scale environmental flow, the neutral 
%This section presents a benchmark problem from Owen et al. (2019) corresponding to a large-scale environmental flow, the neutral 
ABL flow over a flat terrain. The Reynolds number here is $Re=6.62e8$ or $Re_\tau=2.98e7$, which makes the use of wall modeling imperative.
This is also a very good test case for the assessment of wall-modeling approaches at coarse resolutions. The size of the
computational domain is $L_z = H = 1000m$ in the vertical direction and $L_x = L_y = 3 L_z$ in the tangential
directions. The effective resolution in the computational grids used varied between 40 and -88 points in the vertical direction
and 240 to 528 in each of the two spanwise directions. 
Periodic boundary conditions are imposed in the streamwise and spanwise directions. A stress-free condition is imposed at 
the upper boundary, and a zero normal velocity imposed at the bottom and top boundaries. The logarithmic law is used to model 
the wall layer at the bottom boundary
\begin{equation}
u(z)=\frac{u_\tau}{\kappa} \ln \left(\frac{z+z_0}{z_0}\right).
\label{eqn.loglaw_neutral}
\end{equation}
\noindent
The values chosen for the friction velocity and roughness length are $u_\tau = 0.45m/s$ and $z_0 = 0.1m$, respectively. 
Statistics are collected once the quasi-steady state has been achieved, and the results are averaged in time.

\noindent
The approaches tested for this benchmark problem include the MFEV/SMG approach described in section~\ref{sec.mfev_smg}.
In addition, the global Smagorinsky SGS model was implemented and tested in the same setup. Fig.~\ref{fig.abl_neutral_loglaw}
compares streamwise streamwise velocity profiles with the log-law~(\ref{eqn.loglaw_neutral}), which should be the long-time
solution for this problem. As can be observed, the MFEV/SMG approach converges towards the log-law solution as resolution is 
increased. On the other hand, this is not observed for the global SMG model which seems to not behave correctly approaching the lower wall.

\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.90\textwidth]{./figs/plot_loglaw_MFEV_Smag_lx6_to_lx12_solve_utau_t500_1000.pdf}
  \caption{\label{fig.abl_neutral_loglaw} Horizontally averaged streamwise velocity profiles in log-lin, averaged in time between t=500-1000 using MFEV/SMG with traction boundary conditions.}
\end{figure*}

\noindent
The same behavior is observed when looking at the quantity $\phi(z)=(\kappa z/u_\tau)du/dz$ which close to the lower wall
should be approximately equal to one. From the figure it can be seen that the MFEV/SMG approach (black lines) results in a value of 
$\phi(z) \approx 1$ at least for the bottom 500m of the domain, whereas the global SMG results deviate from this value.
\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.90\textwidth]{./figs/plot_dudz_loglaw_MFEV_Smag_lx6_to_lx12_solve_utau_t500_1000.pdf}
  \caption{\label{fig.abl_neutral_dudz} Comparison of time-averaged LES profiles from MFEV/SMG and global SMG with log-law}
\end{figure*}

\noindent
The convergence of the horizontally and time-averaged fluctuating velocities in the neutral ABL problem with p-refinement 
for MFEV/SMG and global SMG is shown in Fig.~\ref{fig.abl_neutral_fluc}.
\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.90\textwidth]{./figs/plot_fluc_MFEV_Smag_lx6_to_lx12.pdf}
  \caption{\label{fig.abl_neutral_fluc} Convergence of fluctuating velocities in neutral ABL problem with p-refinement for MFEV/SMG and global SMG}
\end{figure*}

\noindent
Some additional tests were performed for the neutral ABL benchmark problem to investigate the convergence behavior.
Specifically, the global SMG model was modified so that the filter length scale along the first row of elements next
to the wall would match the known log-law behavior. Even though the solution did not diverge clost to the lower wall with increasing resolution 
with this modification, the solution quality did not really improve for the global SMG model. 
In addition, long time averaging was performed for both MFEV/SMG and global SMG models to investigate agreement with the 
log-law solution. Finally, the vertical domain height was increased from 1km to 2km to avoid the effect of the stresss-free 
BC imposed at the upper boundary, and it was verified that the log-law agreement extended well beyond 1km in the vertical 
direction in the 2km case.







==> tex/preambl.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Geometry 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{geometry}
%\geometry{left   = 1.0in,
%          right  = 1.0in,
%          top    = 1.0in,
%          bottom = 1.0in}

%\usepackage{moreverb,url}
%\usepackage{amssymb,amsmath,amsfonts}
%\usepackage{graphicx}
%\usepackage{rotating}

\usepackage{setspace}
\usepackage{lipsum}
%\newcommand{\verbatimfont}[1]{\renewcommand{\verbatim@font}{\ttfamily#1}}
\usepackage{epstopdf}
\usepackage{alltt}
\usepackage{color}
\usepackage{multirow}
\usepackage{listings}
\usepackage{wrapfig}
\usepackage{enumitem}

\usepackage{fancyvrb}
\fvset{fontsize=\scriptsize}
%\fvset{fontsize=\footnotesize}
\RecustomVerbatimEnvironment{verbatim}{Verbatim}{}

\usepackage{floatrow}
\floatsetup[table]{capposition=top}
\usepackage{algpseudocode,algorithm,algorithmicx}
%\usepackage{algcompatible}
\usepackage{todonotes}

\usepackage[per-mode=symbol]{siunitx}
\usepackage{pgfplots}
%\pgfplotsset{compat=1.17}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Formats
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{subfigure,pgfplots,epsf,graphicx,color}
%\usepackage{amsmath,amsfonts,amsthm,multirow}

\usepackage{comment}
\usepackage{rotating}
\usepackage{tabularx}
\usepackage{float}

\usepackage{pdfpages}
\usepackage{afterpage}
\usepackage{wrapfig}
\usepackage{microtype}
\usepackage{fullpage}
\usepackage{bm} 
\usepackage{caption} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[colorlinks=true]{hyperref}
\hypersetup{
  colorlinks  = true, %Colours links instead of ugly boxes
  urlcolor    = blue, %Colour for external hyperlinks
  linkcolor   = blue, %Colour of internal links
  citecolor   = blue, %Colour of citations
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% epstopdf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newif\ifpdf
%\ifx\pdfoutput\undefined
%   \pdffalse
%\else
%   \pdfoutput=1
%   \pdftrue
%\fi
%\ifpdf
%   \usepackage[update,prepend]{epstopdf}
%   \DeclareGraphicsRule{.eps}{pdf}{.pdf}{`epstopdf #1}
%   \pdfcompresslevel=9
%\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Style 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\DeclareGraphicsExtensions{.gif,.png,.jpg,.pdf,.tiff,.eps}	

\def\baselinestretch{1.0}
\textwidth 6.5in
\textheight 8.50in
\topmargin -0.15in
\parskip   0.05in
\oddsidemargin 0.0in
\parindent 5ex
\renewcommand{\topfraction}{.95}
\renewcommand{\bottomfraction}{.95}
\renewcommand{\textfraction}{.05}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> tex/sgs.tex <==
 \section{ABL GABLS benchmark and Modeling Approaches}

In this section, we consider the GABLS benchmark problem~\cite{beare06}, a stable ABL 
in which the ground temperature (at $z=0$) is cooler than the air temperature and where 
the ground temperature continues to cool over the duration of the simulation.  
The simulation domain is $\Omega = L_x \times L_y \times L_z =$ 400 m $\times$ 400 m $\times$ 400 m,
with $x$ the streamwise direction, $y$ the spanwise direction, and $z$ the vertical direction.
Simulations are initialized (at $t=0$) with constant velocity in the
streamwise direction equal to geostrophic wind speed of $U=8$ m/s. The initial
potential temperature is 265 K in $0\le z\le 100$ m and linearly increased at
a rate of 0.01 K/m in 100 m $\le z\le 400$ m.  The reference potential
temperature is 263.5 K.  The Reynolds number is $Re= UL_b/\nu$,
where $L_b=100$ m is the thickness of the initial thermal boundary layer and $\nu$ 
is the molecular viscosity, and it is $\approx 50M$, which precludes direct numerical 
simulation (DNS) wherein all turbulent scales are resolved.
An initial perturbation is added to the temperature with an amplitude of 0.1 K
on the potential temperature field for $0 \le z\le 50$ m.

%% For Nek5000/RS, this perturbation consists of a number of prime wavenumbers in the two 
%% horizontal directions (e.g., 13, 23) to mimic a small-scale random noise. A similar
%% perturbation was also tried for the three velocity components with an amplitude
%% of 0.08 m/s but the flow development was very similar to the case with only a
%% potential-temperature initial perturbation. Hence, simulations presented only had 
%% potential-temperature perturbation.

Periodic boundary conditions (BCs) are used in the streamwise and spanwise directions.
At the top boundary, ($z=400$ m), a stress-free, rigid lid is applied for momentum, and
the heat flux for the energy equation is set consistent with the 0.01 K/m temperature
gradient initially prescribed in the upper region of the flow.
At the bottom boundary, we perform simulations with impenetrable traction BCs
for the velocity where the specified shear stress comes from Monin-Obukhov
similarity theory~\cite{monin1954}.  For the energy equation, a heat flux is
applied that is derived from the same theory and a specified potential
temperature difference between the flow at a height, $z_1$, and the surface.
The surface temperature is from the GABLS specification following the rule
$\theta_b(t) = 265 - 0.25 t$, where $t$ is in hours.  Because the boundary
conditions are periodic (lateral), or the mass flow rate through the boundaries
is zero (top and bottom),  pressure boundary conditions are not needed.

\subsection{Nek5000/RS LES models}

The traction boundary condition is used in Nek5000/NekRS at the bottom boundary 
representing the lower wall.
   Zero value for the normal velocity component together with traction BCs for the two horizontal
       velocity components and heat flux BCs for the potential temperature, based on the log-law.

In addition, we have explored several SGS modeling approaches
used for this benchmark problem based on high-pass filter (HPF)~\cite{Stolz_Schlatter_2005}, 
mean-field eddy viscosity (MFEV)~\cite{sullivan94}, 
and Smagorinsky (SMG)~\cite{smagor63} with traction BCs summarized as
        (1) HPF SGS model,
        (2) MFEV (SGS for anisotropic part) + HPF (SGS for isotropic), and              
        (3) MFEV (SGS for anisotropic part) + SMG (SGS for isotropic).  
 
\subsubsection{HPF SGS model + traction BCs}
Traction boundary conditions were also used in conjunction with the HPF SGS model for the reduced $Re$ of 50k. 
In this case, following~\cite{Grotjans_Menter1998} and~\cite{Kuzmin_2007}, the boundary of the computational domain 
is not located exactly at the wall, i.e. at $z=0$, but at a finite distance from the wall corresponding to a fixed value 
of $z_1^+=z_1/z_0$, which for $Re=50k$ was set to a value below 5, typically $z_1^+=2$.
Strictly speaking, this implies that a boundary layer of width $z_1$ (corresponding to the specified value of $z_1^+$) should
be removed from the computational domain; however, it is assumed that this width is very small at high Reynolds numbers
and can be considered negligible, so that the equations can be solved in the whole domain with traction BCs prescribed
on the lower boundary. Since the choice of $z_1^+$ is rather arbitrary, we have found that values of $z_1^+$ up
to $5$ produce averaged results that did not differ significantly. 
%%% This can be observed in Fig.~\ref{fig.nek_bc}, which
%%% demonstrates the convergence in comparison between no-slip and traction boundary conditions.
%%% where the horizontally averaged streamwise and spanwise velocity profiles are shown at $t=7h$ for the cases of  no-slip and 
%%% traction BCs at $Re=50k$. The good agreement of traction BCs with noslip is due to the fact that for this $Re$, $z_1^+<5$
%%% is located inside the viscous sublayer and not inside the log-law. This implies that using traction BCs at this $Re$ 
%%% effectively resolves the lower wall BL and cannot lead to asymptotically Reynolds independent results, similar to noslip.

%\begin{figure*}[!t]
%  \centering
%  \includegraphics[width=0.90\textwidth]{./figs/plot_all_mean_u_v_7h_8h_noslip_traction.pdf}
%  \caption{\label{fig.noslip_traction} Horizontally averaged streamwise and spanwise velocities at t=7h and t=8h using 
%      Nek5000 with noslip and traction boundary conditions at two different resolutions, for grid spacing of 3.125m and 1.56m.}
%\end{figure*}


%The traction BC is newly
%implemented into Nek5000 code and experimented together with the no-slip BC
%in comparison for the GABLS1 problem. 
%
%We considered two different resolutions on horizontal direction
%but keeping same reolution in the vertial direction using the total number of grid points,
%$n=64\times 64 \times \times 80$ and $n=256\times 256 \times 80$ which represent
%$8^2$ and $32^2$ elements on the horizontal direction with the polynomial degree of $N=8$.
%The minimum element size in $z$ is 6.10764m and thus the minimum averaged grid spacing is 0.7634m.
%We observe a good agreement of the results between traction and no-slip BCs and thus
%our results in the following sections using the similar rnage of resolutions
%are performed with the choice of no-slip BC.
%






\subsubsection{MFEV (SGS for anisotropic part) + HPF (SGS for isotropic) + traction BCs}
\label{sec.mfev_hpf}
In the efforts described in this subsection, the implementation of the traction BCs for the horizontal velocity 
components is also performed in the context of the log-law for which we follow the approach of ~\cite{Grotjans_Menter1998} 
and~\cite{Kuzmin_2007}, which is appropriate for finite element methods based on a weighted residual formulation.
The normal component of the velocity is set to zero and the traction BCs imposed on the tangential velocity are based 
on the horizontally-averaged slip velocity that develops at the boundary.

The SGS modeling is based on~\cite{sullivan94}, where the SGS stress tensors $\tau^{sgs}_{ij}$ and $\tau^{sgs}_{\theta j}$ 
are expressed in terms of a non-isotropic, mean-field eddy viscosity (MFEV) obtained by the horizontally-averaged mean 
strain rate, and an isotropic, fluctuating part. The law of the wall is effected through the use of the mean-field eddy 
viscosity concept and the approach originally used by~\cite{SCHUMANN1975376} is used to convert the horizontally-averaged 
traction to local values based on the local slip velocity in each of the horizontal directions.
Here, the fluctuating (isotropic) part is taken into account through the use of a high-pass filter filter 
(HPF)~\cite{Stolz_Schlatter_2005}, which is not eddy-viscosity based. In this case, the SGS model of~\cite{sullivan94} 
is based on the following expression
\begin{equation}
\tau^{sgs}_{i j}=-2 \nu_{T}\left\langle S_{i j}\right\rangle,
\label{eqn.tijdef1}
\end{equation}
where the angle brackets $\left\langle \ \ \right\rangle$ denote averaging over the
homogeneous directions and $\nu_T$ is an average eddy viscosity which is expressed in
terms of mean flow quantities. 

In this case, the modified right-hand sides of the NS and energy equations 
(\ref{eq:ns})--(\ref{eq:energy}) are as follows:
\begin{eqnarray}
 \label{eq:ns2}
  \frac{\partial \bar{u}_{i}}{\partial t}
  +\bar{u}_{j}\frac{\partial \bar{u}_{i}}{\partial x_{j}}
  & = & -\frac{\partial \bar{p}}{\partial x_{i}}-\pp{\tau_{ij}}{x_j}
        -2 \epsilon_{i3k} \Omega \bar{u}_k %\nonumber \\
   +  (1-\delta_{i3}) \frac{\partial }{\partial z}\nu_{T} 
   \frac{\partial\langle \bar{u}_i\rangle}{\partial z} - \frac{\theta^{\prime}}{\theta_0} g_i  \\ %\label{eq:inc_filt}
  & \approx & -\frac{\partial \bar{p}}{\partial x_{i}}
        + \frac{1}{\operatorname{Re}} \frac{\partial^{2} 
          \bar{u}_{i}}{\partial x_{j} \partial x_{j}}
        -\chi H_{N} * \bar{u}_{i} % \nonumber\\
   -  2 \epsilon_{i3k} \Omega \bar{u}_k + (1-\delta_{i3}) 
      \frac{\partial }{\partial z}\nu_{T} \frac{\partial\langle \bar{u}_i \rangle}{\partial z} 
   - \frac{\theta^{\prime}}{\theta_0} g_i, \quad\quad
  \\
%\end{eqnarray} 
%\begin{eqnarray}
\label{eq:inc_filt2}
  \frac{\partial \bar{\theta}}{\partial t}
  + \bar{u}_{j}\frac{\partial \bar{\theta}}{\partial x_{j}}
  %&=& -\pp{\tau_{\theta j}}{x_j} \\
    \label{eq:energy_filt2}
  &\approx& \frac{1}{\operatorname{Pe}}
      \frac{\partial^{2} \bar{\theta}}{\partial x_{j} \partial x_{j}}-\chi H_{N} * \bar{\theta} %%\nonumber \\
   + \frac{\partial }{\partial z}\nu_{T} \frac{\partial\langle \bar{\theta} \rangle}{\partial z}.
\end{eqnarray}
%where $\bar{u}_{i}$ and $\bar{p}$ are the grid-filtered velocity and 
%pressure, respectively.  The modeled equations are solved together with
%the incompressbility constraint.

The expression for the MFEV $\nu_T$ is derived so that the law-of-the-wall behavior
can be recovered in the absence of any resolved turbulence as explained below.
According to~\cite{sullivan94}, a model consistent with this idea is as follows:
\begin{equation}
\nu_{T}=\left(C_{K} L_{m}\right)^{2} \sqrt{2\left\langle S_{i j}\right\rangle\left\langle S_{i j}\right\rangle},
 \label{eqn.nuT1}
\end{equation}
where $S_{i j}$ is the strain rate tensor, $C_K$ is a constant and $C_K L_m$ is a mixing-lqength scale.
Equation~(\ref{eqn.nuT1}) simplifies to
\begin{equation}
\nu_{T}=\left(C_{K} L_{m}\right)^{2} \sqrt{\left(\frac{\partial\langle u\rangle}{\partial z}\right)^{2}+\left(\frac{\partial\langle v\rangle}{\partial z}\right)^{2}},
\label{eqn.nuT2}
\end{equation}
and by ignoring the mean wind turning with height at the first grid point implies that the
wind-speed derivative is:
\begin{equation}
\sqrt{\left(\frac{\partial\langle u\rangle}{\partial z}\right)^{2}+\left(\frac{\partial\langle v\rangle}{\partial z}\right)^{2}} \approx \frac{\partial U_{s}}{\partial z},
\label{eqn.dUdz1}
\end{equation}
where $U_{s}$ is the average surface layer wind speed (i.e., $U_{s}=\left\langle\sqrt{u^{2}+v^{2}}\right\rangle$).
The choice of $C_K L_m$ is guided by the need to match Monin-Obukhov similarity theory in the
wall region and the expression. In this theory, the wind-speed derivative becomes
\begin{equation}
\frac{\partial U_{s}}{\partial z}=\frac{u_{\tau} \phi_{m}}{\kappa z},
\label{eqn.dUdz2}
\end{equation}
where $u_{\tau}$ is the friction velocity, $\kappa$ the von Karman constant, $\phi_{m}$ the Monin-Obukhov stability
function for momentum.
Following~\cite{sullivan94}, in order to make use of Equation~(\ref{eqn.nuT1}) we further impose a "constant flux",
traction-type boundary condition at $z=z_{1}$, which states that the sum of the SGS and resolved momentum fluxes be
equal to the surface stress, i.e.,
\begin{equation}
\left[\left\langle\tau^{sgs}_{u w}\right\rangle^{2}+\left\langle\tau^{sgs}_{v w}\right\rangle^{2}\right]^{1 / 2}
 +\left[\langle u w\rangle^{2}+\langle v w\rangle^{2}\right]^{1 / 2}=u_{\tau}^{2} .
\label{eqn.stress}
\end{equation}

As described in section~\ref{s:tractionBC}, this traction boundary condition in Nek is imposed at the
first grid point in the vertical direction, which is assumed to be a point inside the log-layer at a location $z=z_1$,
where the boundary condition for the vertical velocity component is defined to be zero.
For this reason the second term in equation~(\ref{eqn.stress}) corresponding to the resolved momentum fluxes is
identically equal to zero.
In~\cite{sullivan94}, a predictive relationship for the mean-field eddy-viscosity
at the first grid point $z_1$, $\nu_T^\star=\nu_T(z_1)$, is obtained by invoking the approximation
that the fluctuating components of strain are neglected compared to the mean strain so
that only the horizontally-averaged SGS stress in Equation~(\ref{eqn.tijdef1}) is retained.
This leads to
\begin{equation}
\begin{aligned}
%\left\langle\tau_{u w}\right\rangle &=-\left(\left\langle\nu_{t} \gamma\right\rangle+\nu_{T}\right) \frac{\partial\langle u\rangle}{\partial z} \\
%\left\langle\tau_{v w}\right\rangle &=-\left(\left\langle\nu_{t} \gamma\right\rangle+\nu_{T}\right) \frac{\partial\langle v\rangle}{\partial z}
\left\langle\tau^{sgs}_{u w}\right\rangle &=-\nu_{T} \frac{\partial\langle u\rangle}{\partial z}, \\ 
\left\langle\tau^{sgs}_{v w}\right\rangle &=-\nu_{T} \frac{\partial\langle v\rangle}{\partial z}.
\label{eqn.tijsim}
\end{aligned}
\end{equation}
Upon substitution of Equation~(\ref{eqn.tijsim}) into Equation~(\ref{eqn.stress}) and making use of Equations
~(\ref{eqn.dUdz1}) and~(\ref{eqn.dUdz2}), the expression for the mean-field eddy-viscosity, $\nu_T^\star$, for Nek
becomes
\begin{equation}
%\nu_{T}^{\star}=\frac{u_{\tau} \kappa z_{1}}{\phi_{m}\left(z_{1}\right)}-\left\langle\nu_{t} \gamma\right\rangle-\frac{\kappa z_{1}}{u_{\tau} \phi_{m}\left(z_{1}\right)}\left[\langle u w\rangle^{2}+\langle v w\rangle^{2}\right]^{1 / 2}
\nu_{T}^{\star}=\frac{u_{\tau} \kappa z_{1}}{\phi_{m}\left(z_{1}\right)}.
\label{eqn.nuTsim}
\end{equation}

Equation~(\ref{eqn.nuTsim}) provides an adaptive method for estimating the mean-field eddy
viscosity needed to force the computed wind speed derivative to match with
similarity theory at $z = z_1$. At any other height, similar to~\cite{sullivan94}, we use
\begin{equation}
\nu_{T}=\nu_{T}^{\star} \frac{\kappa z_{1}}{u_{\tau} \phi_{m}\left(z_{1}\right)} \sqrt{2\left\langle S_{i j}\right\rangle\left\langle S_{i j}\right\rangle},
 \end{equation}
which follows directly from Equations~(\ref{eqn.nuT1}), ~(\ref{eqn.dUdz1}), and~(\ref{eqn.dUdz2}).
In contrast to~\cite{sullivan94}, a similar correction was also applied to the SGS potential temperature
field, and $\tau^{sgs}_{\theta z}$ becomes:
\begin{equation}
\left\langle\tau^{sgs}_{\theta z}\right\rangle =-\nu_{T} \frac{\partial\langle \theta \rangle}{\partial z}.
\label{eqn.tautheta}
\end{equation}

% Traction BCs
%The implementation of this boundary
%condition in Nek5000/RS is performed using the full stress formulation~\cite{LeeHo1989} and allows also for
%boundaries that are curved and not alligned with any of the axes. The evaluation of the local momentum flux used
%for the traction BCs is described in detail in Section~\ref{s:tractionBC}.
Following~\cite{Grotjans_Menter1998} and~\cite{Kuzmin_2007}, as was already described in the previous subsection, in our approach 
the boundary of the computational domain
is not located exactly at the wall but at a finite distance from the wall corresponding to a fixed value of $z_1^+=z/z_0$.
Strictly speaking, this implies that a boundary layer of width $z_1$ (corresponding to the specified value of $z_1^+$) should
be removed from the computational domain; however, it is assumed that this width is very small at high Reynolds numbers
and can be considered negligible, so that the equations can be solved in the whole domain with traction BCs prescribed
on the lower boundary. Since the choice of $z_1^+$ is rather arbitrary, we have found that values of $z_1^+$ up
to $10$ at the target $Re$ produce averaged results that do not differ significantly.

Results obtained with the MFEV/HPF approch led to converged results with increasing resolution. 
Fig.~\ref{fig.mfev_hpf} shows horizontally averaged profiles of streamwise and spanwise velocities
which are also averaged in time between t=8h and t=9h, and demostrates convergence with increasing
resolution.
\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.9\textwidth]{./figs/plot_Nek_ncarBC_Re50M_convergence_8h_9h_u_v.pdf}
  \caption{\label{fig.mfev_hpf} Horizontally averaged streamwise and spanwise velocities between t=8h and t=9h using 
      Nek5000 with MFEV/HPF and traction boundary conditions at three different resolutions.}
\end{figure*}
Moreover, the obtained profiles were almost identical for different values of $Re$, as well as 
of $z_1^+$ as can be observed in Fig.~\ref{fig:nek_vis}, left and right, respectively.
\begin{figure*}[!h]
  \begin{center}
     \includegraphics[width=0.5\textwidth]{./figs/plot_Nek_ncarBC_Re50M_vs_Re5M_7h_8h.pdf}
     \hspace{-2em} 
     \includegraphics[width=0.5\textwidth]{./figs/plot_Nek_ncarBC_z10_vs_z5_7h_8h.pdf}
   \caption{\label{fig:nek_vis} Convergence of MFEV/HPF approach with Re and $z_1^+$.}
  \end{center}
\end{figure*}

\subsubsection{MFEV (SGS for anisotropic part) + SMG (SGS for isotropic) + traction BCs}
\label{sec.mfev_smg}
In this subsection, the sub-grid-scale dissipation is again effected through a non-isotropic, 
mean-field eddy viscosity (MFEV) obtained by the horizontally-averaged mean strain rate, and an 
isotropic, fluctuating part, which is here taken into account through a Smagorinsky (SMG) model 
based on the fluctuating strain rate. In this case, the SGS model of~\cite{sullivan94}
is based on the following expression
\begin{equation}
\tau^{sgs}_{i j}=-2 \gamma \nu_t S_{i j} -2 \nu_{T}\left\langle S_{i j}\right\rangle,
\label{eqn.tijdef2}
\end{equation}
where also here the angle brackets $\left\langle \ \ \right\rangle$ denote averaging over the
homogeneous directions and $\nu_T$ is an average eddy viscosity which is expressed in
terms of mean flow quantities. In Eq.~(\ref{eqn.tijdef2}) $\gamma$ is
an ``isotropy factor,'' which accounts for variability in the SGS constants due to
anisotropy of the mean flow. In~\cite{sullivan94}, the fluctuating eddy viscosity,
$\nu_t$, is obtained using an eddy viscosity model based on the SGS turbulent kinetic
energy equation, in which the shear production term is computed from the fluctuating
velocities as suggested by~\cite{Schumann1975}.
%For the former model, which is not eddy-viscosity based, $\nu_t$ in
%Eq.~(\ref{eqn.tijdef2}) is by definition equal to zero.

When the fluctuating (isotropic) part of turbulent motion is taken into account through the use of
a SMG model based on the fluctuating strain rate, which is eddy-viscosity based,
$\nu_t$ in Eq.~(\ref{eqn.tijdef2}) is non-zero and the full stress tensor has to be taken into
account.

\begin{eqnarray}
 \label{eq:ns3}
  \frac{\partial \bar{u}_{i}}{\partial t}
  +\bar{u}_{j}\frac{\partial \bar{u}_{i}}{\partial x_{j}}
  & = & -\frac{\partial \bar{p}}{\partial x_{i}}-\pp{\tau_{ij}}{x_j}
        -2 \epsilon_{i3k} \Omega \bar{u}_k %%\nonumber \\
    +  (1-\delta_{i3}) \frac{\partial }{\partial z}\nu_{T} 
   \frac{\partial\langle \bar{u}_i\rangle}{\partial z} - \frac{\theta^{\prime}}{\theta_0} g_i \quad  \\ %\label{eq:inc_filt}
  & \approx & -\frac{\partial \bar{p}}{\partial x_{i}}
        + \frac{\partial}{\partial x_j} \left(\frac{1}{\operatorname{Re}} +\gamma \nu_t \right) 
          2S^n_{ij} - 2 \epsilon_{i3k} \Omega \bar{u}_k %%\nonumber\\
    +   (1-\delta_{i3}) 
      \frac{\partial }{\partial z}\nu_{T} \frac{\partial\langle \bar{u}_i \rangle}{\partial z} - \frac{\theta^{\prime}}{\theta_0} g_i, \quad
\\
%\end{eqnarray} \label{eq:inc_filt3}
%\begin{eqnarray}
  \frac{\partial \bar{\theta}}{\partial t}
  + \bar{u}_{j}\frac{\partial \bar{\theta}}{\partial x_{j}}
  %&=& -\pp{\tau_{\theta j}}{x_j} \\
    \label{eq:energy_filt3}
  &\approx& \frac{\partial }{\partial x_{j}} \left(\frac{1}{\operatorname{Pe}} 
   +\frac{\gamma \nu_t}{Pr_t} \right) \frac{\partial \bar{\theta}}{\partial x_{j} } 
   + \frac{\partial }{\partial z}\nu_{T} \frac{\partial\langle \bar{\theta} \rangle}{\partial z}.
\end{eqnarray}

Here again, the expression for $\nu_T$ is derived so that the law-of-the-wall behavior
can be recovered in the absence of any resolved turbulence, in the same way as explained in the previous 
subsection~\ref{sec.mfev_hpf}.

On the other hand, for the isotropic part of the eddy viscosity $\nu_t$, the fluctuating strain rate is used:
\begin{equation}
\nu_t=\left(C_s \Delta\right)^2 \sqrt{2 S^{\prime}_{i j} S^{\prime}_{i j}},
\end{equation}
where 
\begin{equation}
S^{\prime}=\sqrt{2\left\langle\left(S_{i j}-\left\langle S_{i j}\right\rangle\right)\left(S_{i j}-\left\langle S_{i j}\right\rangle\right)\right\rangle},
 \end{equation}
and
\begin{equation}
C_s=\left(C_k \sqrt{\frac{C_k}{C_\epsilon}}\right)^{1 / 2}.
\end{equation}
The isotropy factor $\gamma$ is obtained by
\begin{equation}
\gamma=\frac{S^{\prime}}{S^{\prime}+\langle S\rangle},
\end{equation}
and where 
\begin{equation}
\langle S\rangle=\sqrt{2\left\langle S_{i j}\right\rangle\left\langle S_{i j}\right\rangle}.
\end{equation}
%\begin{equation}
%\nu_t \gamma=\left(\hat{C}_s \Delta\right)^2 \sqrt{2 S_{i j} S_{i j}}
%\end{equation}
%
%\begin{equation}
%\hat{C}_s=C_s \sqrt{\gamma}
%\end{equation}
Finally, the expression that holds for the horizontally averaged traction along the lower wall differs from~(\ref{eqn.tijsim}) 
because $\nu_t$ is not zero along the lower wall, and is:
\begin{equation}
\begin{aligned}
\left\langle\tau_{u w}\right\rangle &=-\left(\left\langle\nu_t \gamma\right\rangle+\nu_T\right) \frac{\partial\langle u\rangle}{\partial z}, \\ 
\left\langle\tau_{v w}\right\rangle &=-\left(\left\langle\nu_t \gamma\right\rangle+\nu_T\right) \frac{\partial\langle v\rangle}{\partial z}.
\end{aligned}
\end{equation}

Results obtained with the MFEV/SMG approch also demonstrate convergence with increasing resolution
as well as asymptotic convergence with $Re$ and $z_1^+$. Moreover, convergence with resolution
seems to be faster with MFEV/SMG as compared with the MFEV/HPF approach described in the previous subsection.
This can be observed in Fig.~\ref{fig.mfev_smg}, which shows horizontally averaged streamwise and spanwise velocities 
at t=6h, t=7h and t=8h using MFEV/SMG and traction boundary conditions at the lowest two resolutions, which can be 
compared to Fig.~\ref{fig.mfev_hpf}.

\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.90\textwidth]{./figs/plot_smag_128_256_6h_7h_8h.pdf}
  \caption{\label{fig.mfev_smg} Horizontally averaged streamwise and spanwise velocities at t=6h, t=7h and t=8h using 
      Nek5000 with MFEV/SMG and traction boundary conditions at two different resolutions.}
\end{figure*}

Fig.~\ref{fig.mfev_smg_hpf} shows the horizontally averaged streamwise and spanwise velocities at t=6h for the two
highest resolutions $512^3$ and $1024^3$ for MFEV/HPF and for $512^3$ for MFEV/SMG and AMR-Wind, respectively. As can
be observed, both Nek5000/NekRS approaches converge to the same profiles as resolution is increased; they also agree
well with the AMR-Wind obtained profiles at $512^3$.
\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.90\textwidth]{./figs/plot_smag_vs_hpf_128_256_512_t1700.pdf}
  \caption{\label{fig.mfev_smg_hpf} Horizontally averaged streamwise, spanwise velocities at t=6h using MFEV/SMG and MFEV/HPF 
      with traction boundary conditions, compard with AMR-Wind results, for $512^3$.}
\end{figure*}

Good convergence is also observed in second order quantities, as can be observed in Fig.~\ref{fig.mfev_fluc_256_512} 
(top and bottom), for resolutions $256^3$ and $512^3$, respectively. The resolved fluctuations obtained by 
the two approaches MFEV/HPF and MFEV/SMG compare reasonably well with AMR-Wind obtained results for the same effective resolution.
Finally, according to~\cite{sullivan94}, the mean-field eddy viscosity $\nu_T$ and isotropy factor $\gamma$ play important 
roles near the lower wall where mean shear is large. Away from the wall in the middle of the ABL, the fluctuating resolved 
strain should be almost a factor of 10 larger than the mean strain for typical grid resolutions used. In this region, 
$\nu_T \ll \nu_t$ and $\gamma \rightarrow 1$. For this reason, they suggest that for $z > z_i/2$, where $zi$ is the depth of 
the ABL ($\approx 200$), $\gamma$ should be set to $1$ and $\nu_T$ to 0. Forcing this at lower resolutions, e.g. for $256^3$ 
removes a bump which appears in the streamwise fluctuation profile between $z=100$ and $200$, as can be seen in 
Fig.~\ref{fig.mfev_fluc_256_512}.

\begin{figure*}%[!t]
  \begin{center}
     \includegraphics[width=0.8\textwidth]{./figs/plot_Nek_Smag_AMR_ncarBC_convergence_7h_9h_fluc_256.pdf}
     \\
     \includegraphics[width=0.8\textwidth]{./figs/plot_Nek_Smag_AMR_ncarBC_convergence_7h_9h_fluc_512.pdf}
   % \includegraphics[width=0.48\textwidth]{./figs/plot_Nek_Smag_AMR_ncarBC_convergence_7h_9h_fluc_256.pdf}
   % \includegraphics[width=0.48\textwidth]{./figs/plot_Nek_Smag_AMR_ncarBC_convergence_7h_9h_fluc_512.pdf}
   \caption{\label{fig.mfev_fluc_256_512} Horizontally averaged streamwise, spanwise and vertical resolved fluctuation velocities 
      time-averaged between t=7h and t=9h using MFEV/SMG and MFEV/HPF with traction boundary conditions, compard with AMR-Wind 
      results, for $256^3$ (top) and $512^3$ (bottom).}
  \end{center}
\end{figure*}

%\begin{figure*}[!t]
%  \centering
%  \includegraphics[width=0.80\textwidth]{./figs/plot_Nek_Smag_AMR_ncarBC_convergence_7h_9h_fluc_256.pdf}
%  \caption{\label{fig.mfev_fluc_256} Horizontally averaged streamwise, spanwise and vertical resolved fluctuation velocities 
%      time-averaged between t=7h and t=9h using MFEV/SMG and MFEV/HPF with traction boundary conditions, compard with AMR-Wind 
%      results, for $256^3$.}
%\end{figure*}
%
%\begin{figure*}[!b]
%  \centering
%  \includegraphics[width=0.80\textwidth]{./figs/plot_Nek_Smag_AMR_ncarBC_convergence_7h_9h_fluc_512.pdf}
%  \caption{\label{fig.mfev_fluc_512} Horizontally averaged streamwise, spanwise and vertical resolved fluctuation velocities 
%      time-averaged between t=7h and t=9h using MFEV/SMG and MFEV/HPF with traction boundary conditions, compard with AMR-Wind 
%      results, for $512^3$.}
%\end{figure*}

Figure~\ref{fig:mean} shows profiles of the horizontally-averaged streamwise,
$\left< u \right>$, and spanwise, $\left< v \right>$, wind velocities (top) and
potential temperature, $\left< \theta \right>$, (bottom) at 1-hour time
intervals between 1 h--10 h for a mesh resolution of $n=512^3$ ($\dx= 0.78$ m)
for each code.  The left figures show NekRS results using MFEV and HPF, the
center figures show NekRS using MFEV and Smagorinsky, and the right figures
show the results for AMR-Wind.  As can be observed, the time evolution of the
mean velocity and temperature profiles obtained from the two codes agree quite
well despite using very different numerical methods and subgrid scale models.
The agreement between AMR-Wind and NekRS improves when using MFEV and
Smagorinsky (i.e., between the center and right figures).  Specifically, the
height of the low level jet peak velocity during quasi-steady evolution in the
GABLS problem (after approximately 7 h) is between $150$ and $160$ m, and its
maximum value is between $9.5$ and $9.7$ m/s. An outgrowith of these comparative
simulations has been a concerted effort to carefully validate and cross-check
the SGS models.  The improvement in the NekRS SGS model, realized by moving
away from the HPF model to using the Smagorinsky model for the isotropic stress
term, is a direct outcome of this collaborative effort.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
  \begin{center}

%{\setlength{\unitlength}{1.0in}
     \includegraphics[width=0.35\textwidth]{./figs/nek_hpf_mfev_trac_512_uv.png}
     \hspace{-2em}
     \includegraphics[width=0.35\textwidth]{./figs/nek_smg_mfev_trac_512_uv.png}
     \hspace{-2em}
     \includegraphics[width=0.35\textwidth]{./figs/amr_smg_trac_512_uv.png}
     \\
     \hspace{-2em}
     \includegraphics[width=0.35\textwidth]{./figs/nek_hpf_mfev_trac_512_t.png}
     \hspace{-2em}
     \includegraphics[width=0.35\textwidth]{./figs/nek_smg_mfev_trac_512_t.png}
     \hspace{-2em}
     \includegraphics[width=0.35\textwidth]{./figs/amr_smg_trac_512_t.png}
     \hspace{-2em}
%  \begin{picture}(6.500,0.00)(0,0)
%     \put(0.61,2.83){\Large $\left< v \right>$}
%     \put(1.10,2.83){\Large $\left< u \right>$}
%     \put(1.05,1.20){\Large $\left< \theta \right>$}
%  \end{picture}}
   \caption{\label{fig:mean}NekRS (HPF, SMG) and AMR-Wind:
     velocity magnitude and potential temperature at each hour, 1 h, 2 h,...,9 h.
     }
  \end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{AMR-Wind LES model} %%%% -- {\color{blue}Mike B, Matt}}
AMR-Wind can use either an algebraic [CITE] or one-equation [CITE]
subgrid-scale turbulence model for performing LES.  In both cases, the stress
tensor in (\ref{eq:ns}) is defined following the Boussinesq
turbulence closure approximation as
\begin{equation}
   \label{eq:tau_SGS}
   \tau_{ij} = -\left(\nu + \nu_{SGS}\right) \left( \frac{\partial \bar{u}_{i}}{\partial x_j} + \frac{\partial \bar{u}_{j}}{\partial x_i}\right) + \frac{2}{3}k_{SGS} \delta_{ij}\,
\end{equation}
where $\nu$ is the molecular viscosity and $\nu_{SGS}$ and $k_{SGS}$ are the
subgrid-scale turbulent viscosity and kinetic energy, respectively.  In
practice, we compute the deviatoric part and absorb the isotropic part, $2/3
k_{SGS} \delta_{ij}$ into the modified pressure.  Likewise, the potential
temperature flux found in Eq.~(\ref{eq:energy}) is defined as
\begin{equation}
   \label{eq:q_SGS}
   \tau_{\theta j} = -\left( \frac{\nu}{\textrm{Pr}} +  \frac{\nu_{SGS}}{\textrm{Pr}_t} \right) \frac{\partial \theta}{\partial x_j}\,,
\end{equation}
where $\textrm{Pr}$ and $\textrm{Pr}_t$ are the laminar and turbulent Prandtl
numbers.  In our case, $\textrm{Pr}_t$ is sensitive to thermal stratification
where, under unstable to neutral stratification, it takes a value of $1/3$, but
it smoothly transitions to a value of one in stable stratification.

In the work presented here, we use the standard algebraic subgrid-scale model
of Smagorinsky which gives $\nu_{SGS}$ as
\begin{equation}
   \label{eq:Smagorinsky}
   \nu_{SGS} = \left( C_s \Delta \right)^2 \left( \bar{S}_{ij} \bar{S}_{ij} \right)^{1/2}\,,
\end{equation}
where $C_s=0.135$ is a model constant, $\Delta$ is a lengthscale set
to the cube-root of the computational-grid-cell volume, and $S_{ij}$ is the
strain-rate tensor defined as
\begin{equation}
   \label{eq:Sij}
   \bar{S}_{ij} = \frac{1}{2}\left(\frac{\partial \bar{u}_{i}}{\partial x_j} + \frac{\partial \bar{u}_{j}}{\partial x_i}\right)\,.
\end{equation}
As with Nek5000/RS, although this flow is of extremely high Reynolds number,
the $\nu_{SGS}$ is orders of magnitude greater than $\nu$, and when inserting
the stress tensor or potential temperature flux vector of
Eq.~(\ref{eq:tau_SGS}) and Eq.~(\ref{eq:q_SGS}) into Eqs.~(\ref{eq:ns})-(\ref{eq:energy}),
the flow has an effectively much lower Reynolds number and becomes a tractable
numerical problem with proper drain of turbulent energy at the grid resolution
which dictates the subgrid-scale model lengthscale, $\Delta$.




==> tex/statistics.tex <==


 \subsection{Statistics}

  -- Ananias ??

  -- Matt ??

